D2D Assisted Beamforming for Coded Caching

Device-to-device (D2D) aided beamforming for coded caching is considered in finite signal-to-noise ratio regime. A novel beamforming scheme is proposed where the local cache content exchange among nearby users is exploited. The transmission is split into two phases: local D2D content exchange and downlink transmission. In the D2D phase, users can autonomously share content with the adjacent users. The downlink phase utilizes multicast beamforming to simultaneously serve all users to fulfill the remaining content requests. We first explain the main procedure via two simple examples and then present the general formulation. Furthermore, D2D transmission scenarios and conditions useful for minimizing the overall delivery time are identified. We also investigate the benefits of using D2D transmission for decreasing the transceiver complexity of multicast beamforming. By exploiting the direct D2D exchange of file fragments, the common multicasting rate for delivering the remaining file fragments in the downlink phase is increased providing greatly enhanced overall content delivery performance.

==> complexity_analyze.tex <==
%!TeX root = d2d-cc.tex
\section{complexity reduction in beam design}
\label{sec:complexity_analyze}
So far we have shown the effects of D2D transmission in the per user rate. Lets investigate the effects of D2D in decreasing the MAC conditions in optimization problem. As we mentioned in the previous sections, using D2D transmission in wireless network helps to reduce the complexity for the beamforming. In theorem 1 we introduce two boundaries for the number of MAC conditions.

Theorm 1: Maximum and minimum number of MAC conditions for the DL Phase when $i$ subsets of users have been chosen in D2D transmission are 
%\begin{align}
%   a=&\left\lfloor{\frac{2(\binom{K}{2}-i)}{K}}\right\rfloor,\quad \quad \text{for} \ \ i \leqslant \binom{K}{2} \label{eq:NA1} \\
%    b=&2(\binom{K}{2}-i)-aK,\label{eq:NA2}\\
%    \text{MAC}_\text{min} & =(K-b)*(2^a-1)+b(2^{a+1}-1),\label{eq:NA3}\\
%    X=i & -\binom{U-1}{2}, \ \text{for}\ \binom{U-1}{2} <  i\leqslant \binom{U}{2}\nonumber,\\ U&\leqslant K,\label{eq:NA4} \\
%    Y&=U-(X+1), \label{eq:NA5}\\
%    \text{MAC}_\text{max}&=(K-U)*(2^{K-1}-1)\nonumber\\ +Y&(2^{K-(U-1)}-1)+X(2^{K-U}-1) \label{eq:NA6} \\\nonumber
%    +2&^{K-(X+1)}-1\text{,}
%\end{align}
\begin{align}
    &\text{MAC}^{i}_\text{min} =(t+L-b)(2^a-1)+b(2^{a+1}-1),&\label{eq:NA3}\\
    &a=\left\lfloor{\frac{(t+1)(\binom{t+L}{t+1}-i)}{t+L}}\right\rfloor,\quad  \text{for} \ \ i \leqslant \binom{t+L}{t+1},& \label{eq:NA1} \\
    &b=(t+1)(\binom{t+L}{t+1}-i)-a(t+L),&\label{eq:NA2}\\
    &\text{MAC}^{i}_\text{max}=(t+L-U)(2^{\binom{t+L-1}{t}}-1)+&\nonumber\\&(U-(U_{1}+1))(2^{(\binom{t+L-1}{t}-\binom{U-2}{t})}-1)+& \nonumber \\
    &U_{1}(2^{(\binom{t+L-1}{t}-(\binom{U-2}{t}+\binom{U_{1}-1}{t-1}-Y))}-1)+& \nonumber \\&(2^{\binom{t+L-1}{t}-X}-1)\text{,}& \label{eq:NA6}\\
    &X=i  -\binom{U-1}{t+1}, \ \text{for}\ \binom{U-1}{t+1} <  i\leqslant \binom{U}{t+1}\nonumber,&\\ &U\leqslant (t+L),&\label{eq:NA4} \\
    &\binom{U_{1}-1}{t} <  X\leqslant \binom{U_{1}}{t},& \label{eq:u1} \\
    &Y=\binom{U_1}{t}-X,& \label{eq:NA5}
\end{align}
where $i$ is the number of subsets (time slots) that has been chosen in D2D transmission.

The number of MAC conditions vary between these two boundaries based on which subsets have been chosen for D2D sub-phase. Fig.~\ref{fig:NA1} shows the maximum and minimum number of MAC conditions ($K=10,\ L=9,\ t=1$) for different number of D2D transmissions (the number of time slots). As it can be seen from the figure, the number of MAC conditions can decrease drastically by using just few D2D transmissions, which helps to solve the beamformers much more faster. For the case depicted in the Fig.~\ref{fig:NA1}, by choosing only 5 different subsets of users among 45 different available subsets, the number of MAC conditions can be reduced in half. Therefore, D2D transmission  have a huge gain from the aspect of complexity reduction in beam design.
\begin{figure}
    \centering 
    \includegraphics[width=1\columnwidth,keepaspectratio]{figs/MAC.eps}
    \caption{the normalized number of MAC conditions Vs the number of subsets chosen for D2D transmission for $k=10, \ L=9$ and $t=1$.}
\label{fig:NA1}
\end{figure}

another important factor in beamforming complexity is the number of quadratic parameters in the (SCA). In the next theorem we introduce the boundaries for quadratic equations.

Theorem 2: Maximum and minimum number of quadratic parameters when $i$ subsets of users in D2D sub-phase has been chosen is 
%\begin{align}
%    &V=\binom{K}{2}-i, \label{eq:NA7}\\
%    &A_1=V-(a-1),\nonumber
%    \ \ A_2=V-a,\\ 
%    &B_1=aA_1,
%    \ \ B_2=(a+1)A_2\label{eq:NA8}\\
%    &T_\text{max}= bB_2+(K-b)B_1\label{eq:NA9}\\
%    &A_{1}^{'}=V-(K-2),\ \ \nonumber
%    A_{2}^{'}=V-(K-U),\\ \nonumber
%    &A_{3}^{'}=V-(K-(U+1)),\\ 
%    &A_{4}^{'}=V-(K-(X+2)),\\ \nonumber
%    &B_{1}^{'}=(K-1)A_{1}^{'},\ \ B_{2}^{'}=(K-(U-1))A_{2}^{'},\\
%    &B_{3}^{'}=(K-U)A_{3}^{'}, \ \ \label{eq:NA10} B_{4}^{'}=(K-(X+1))A_{4}^{'},\nonumber\\ 
%    &T_\text{min}=(K-U)B_{1}^{'}+YB_{2}^{'}+XB_{3}^{'}+B_{4}^{'},\label{eq:NA11}
%\end{align}
\begin{align}
    &Q^{i}_\text{max}= bA_2B_2+(t+L-b)A_1B_1&\label{eq:NA9}\\    
    &A_1=a,
    \ \ A_2=a+1,&\\ 
    &B_1=\mathbf{M}^{i}_{\text{T}}-A_1+1,
    \ \ B_2=\mathbf{M}^{i}_{\text{T}}-A_2+1&\label{eq:NA8}\\
    &\mathbf{M}^{i}_{\text{T}}=\binom{t+L}{t+1}-i,& \label{eq:NA7}\\
    &Q^{i}_\text{min}=(t+L-U)A_{1}^{'}B_{1}^{'}+(U-(U_1+1))A_{2}^{'}B_{2}^{'}+& \nonumber\\
    &U_1A_{3}^{'}B_{3}^{'}+A_{4}^{'}B_{4}^{'},&\label{eq:NA11} \\
    &A_{1}^{'}=\binom{t+L-1}{t},\ \ \nonumber
    A_{2}^{'}=A_1^{'}-\binom{U-2}{t},&\\ 
    &A_{3}^{'}=A_{2}^{'}-\binom{U_1-1}{t-1}+Y, \ A_{4}^{'}=A_1^{'}-X,& \\ 
    &B_{1}^{'}=\mathbf{M}^{i}_{\text{T}}-A_{1}^{'}+1,\ \ B_{2}^{'}=\mathbf{M}^{i}_{\text{T}}-A_{2}^{'}+1,&\\
    &B_{3}^{'}=\mathbf{M}^{i}_{\text{T}}-A_{3}^{'}+1, \ \ %\label{eq:NA10}
    B_{4}^{'}=\mathbf{M}^{i}_{\text{T}}-A_{4}^{'}+1,&\nonumber
\end{align}
where $Q^{i}_\text{max}$ is the maximum number of variables in quadratic form and $Q^{i}_\text{min}$ is the minimum number of variables, $\mathbf{M}^{i}_{\text{T}}$ is the total number of massages that is sent by BS after $i$ number of D2D time slots are done. Moreover, $a$ is defined in~\eqref{eq:NA1}, $b$ is defined in~\eqref{eq:NA2}, $X$ and $U$ are defined in~\eqref{eq:NA4}, $U_1$ is defined in \eqref{eq:u1} and $Y$ is defined in~\eqref{eq:NA5}. Finally, $K$ is the number of users and $i$ is the number of subsets that have been used in D2D transmission.
\begin{figure}
    \centering 
    \includegraphics[width=1\columnwidth,keepaspectratio]{figs/quad.eps}
    \caption{normalized number of quadratic variables vs the number of subsets used in D2D transmission. The green curve here corresponds to the red curve in Fig.~\ref{fig:NA1} and the red one here corresponds to the green one in Fig.~\ref{fig:NA1}.}
\label{fig:NA2}
\end{figure}

Fig.~\ref{fig:NA2} depicts the upper and lower boundaries for the same scenario as Fig.~\ref{fig:NA1}. As it can be seen, two boundaries for quadratic variables are almost the same and the gap between these two boundaries is not as huge as MAC conditions. Thus, number of MAC conditions determine the level of complexity for beamforming. Moreover, the role of D2D transmission in the reduction of total number of quadratic variables is huge too; by choosing 13 number of different subsets we can reduce the total number of quadratic variables (for this case) to half, which is a huge gain for complexity reduction of beamforming. 

It is worth to mention that in general we assume that $t+L \leqslant K$, when $t+L$ is less than $K$ we have $\binom{K}{t+L}$ different transmission times. Thus, all the equations in this paper is valid for each of these transmission times. 
%
%It is worth to mention that, we have considered $L=K-1 \ \text{and}\ t=\frac{KM}{N}=1$ in this section, in order to be able to show the benefits of D2D transmission in beamforming in a simple way.

